On the Potential and Limitations of Few-Shot In-Context Learning to Generate Metamorphic Specifications for Tax Preparation Software

Due to the ever-increasing complexity of income tax laws in the United States, the number of US taxpayers filing their taxes using tax preparation software (henceforth, tax software) continues to increase. According to the U.S. Internal Revenue Service (IRS), in FY22, nearly 50% of taxpayers filed their individual income taxes using tax software. Given the legal consequences of incorrectly filing taxes for the taxpayer, ensuring the correctness of tax software is of paramount importance. Metamorphic testing has emerged as a leading solution to test and debug legal-critical tax software due to the absence of correctness requirements and trustworthy datasets. The key idea behind metamorphic testing is to express the properties of a system in terms of the relationship between one input and its slightly metamorphosed twinned input. Extracting metamorphic properties from IRS tax publications is a tedious and time-consuming process. As a response, this paper formulates the task of generating metamorphic specifications as a translation task between properties extracted from tax documents - expressed in natural language - to a contrastive first-order logic form. We perform a systematic analysis on the potential and limitations of in-context learning with Large Language Models(LLMs) for this task, and outline a research agenda towards automating the generation of metamorphic specifications for tax preparation software.

==> emnlp2023-latex/4_model.tex <==
\section{Models Studied}

\subsection{Generation with Simple Prompts}

In the most basic model, we directly prompt an LLM to translate the metamorphic specification to first-order logic.

\subsection{Generation with Explicit Prompts}

We guide the translation by defining predicates manually

\subsection{Automated Construction of Explicit Prompts}

We guide the translation by providing predicates that were automatically generated. Two options: 1) Chaining prompts to an LLM - we first ask questions to obtain candidate predicates, then we prompt for translation. 2) We leverage dependency parses (or other structured NLP representations) to obtain candidate predicates.  

\subsubsection{Chaining Prompts}

\subsubsection{Dependency-parse Guided Prompt Construction}

==> emnlp2023-latex/Prompt-example-new.tex <==

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|}
\hline
n-shots & \multicolumn{1}{c|}{End-to-End} \\ \hline
 & \multicolumn{1}{c|}{-} \\ \hline
0 & \begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
1 & \begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ In this case, the first order predicates are: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Using these predicates, you can generate the following rules in first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
2 & \begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ As another example, \\ Take a look at the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ In this case, the first order predicates are: \\ \\ \\ Blind(x): x is an individual who is blind.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, D): where x and z are equal individuals except differing only by the predicates in set D.\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Blind(x) ∧ EqualExcept(x, y, {Blind}) → Tax(t, x) ≤ Tax(t, y))\\ \\ For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
\end{tabular}%
}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|ll|}
\hline
n-shots & \multicolumn{2}{c|}{Explicit} \\ \hline
 & \multicolumn{1}{c|}{Prompt4Predicate} & \multicolumn{1}{c|}{Prompt4FOL} \\ \hline
0 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ - individual has married filing jointly (MFJ) status \\ - individual has a senior spouse \\ - individual receives tax benefits \\ - individual is similar to another individual \\ - other individual does not have a senior spouse\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
1 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Take a look at the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x): x is an individual who is senior.\\ MarriedFilingJointly(x): x has the married filing jointly status.\\ Tax(t, x): t is the tax paid by individual x.\\ Spouse(x, y): x is the spouse of y.\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
2 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ In a similar fashion, \\ Take a look at the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Blind(x): x is an individual who is blind.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, D): where x and z are equal individuals except differing only by the predicates in set D.\\ \\ In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ Similarly, \\ For the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ Using these predicates, you can generate the following rules in first order logic.\\ \\ \\ ∀x∀y(Blind(x) ∧ EqualExcept(x, y, {Blind}) → Tax(t, x) ≤ Tax(t, y))\\ \\ Take a look at the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this case, the first order predicates are: \\ \\ \\ MFJ(x): x is an individual with the married filing jointly status.\\ SeniorSpouse(y): y is a senior spouse of an individual.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ {MFJ(x), SeniorSpouse(y), Tax(t, x), EqualExcept(x, z, S)}\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \hline
\end{tabular}%
}
\end{table*}

==> emnlp2023-latex/Prompt-example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}|c|l|lc|ll|@{}}
\toprule
n-shots & \multicolumn{1}{c|}{End-to-End} & \multicolumn{2}{c|}{Implicit} & \multicolumn{2}{c|}{Explicit} \\ \midrule
 & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{Prompt4Predicate} & Prompt4FOL & \multicolumn{1}{c|}{Prompt4Predicate} & \multicolumn{1}{c|}{Prompt4FOL} \\ \midrule
0 & \begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & - & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ - individual has married filing jointly (MFJ) status \\ - individual has a senior spouse \\ - individual receives tax benefits \\ - individual is similar to another individual \\ - other individual does not have a senior spouse\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \midrule
1 & \begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ In this case, the first order predicates are: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Using these predicates, you can generate the following rules in first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}For the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & - & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Take a look at the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x): x is an individual who is senior.\\ MarriedFilingJointly(x): x has the married filing jointly status.\\ Tax(t, x): t is the tax paid by individual x.\\ Spouse(x, y): x is the spouse of y.\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \midrule
2 & \begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ As another example, \\ Take a look at the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ In this case, the first order predicates are: \\ \\ \\ Blind(x): x is an individual who is blind.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, D): where x and z are equal individuals except differing only by the predicates in set D.\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Blind(x) ∧ EqualExcept(x, y, {Blind}) → Tax(t, x) ≤ Tax(t, y))\\ \\ For the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate your answer in the following format \\ \\ {your generated predicates}\\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ In this case, the first order predicates are: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ Similarly, \\ Take a look at the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Blind(x): x is an individual who is blind.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, D): where x and z are equal individuals except differing only by the predicates in set D.\\ \\ In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ Now, generate predicates for this statement. \\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & - & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Take a look at the following statement.\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Senior(x) : x is an individual who is senior.\\ Tax(t, x): t is the tax paid by individual x\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ In a similar fashion, \\ Take a look at the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ The first order predicates for this statement would look like: \\ \\ \\ Blind(x): x is an individual who is blind.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, D): where x and z are equal individuals except differing only by the predicates in set D.\\ \\ In the following statement\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this statement, what would the predicates look like?\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the predicates in the following format \\ \\ {your generated predicates} \\ \\ DO NOT generate any other text.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}In the following statement\\ \\ "A senior (over age of 65) must receive similar or better tax benefits when compared to a person without the \\ seniority who is similar in every other aspect (due to higher standard deductions for seniors)."\\ \\ These predicates can be used to generate the following first order logic.\\ \\ \\ ∀x∀y(Senior(x)  ∧ EqualExcept(x,y,{Senior}) → Tax(t,x) ≤ Tax(t,y)\\ \\ Similarly, \\ For the following statement.\\ \\ "A blind individual must receive similar or better tax benefits when compared to a person without the disability \\ who is similar in every other aspect (due to higher standard deductions for blind individuals)."\\ \\ Using these predicates, you can generate the following rules in first order logic.\\ \\ \\ ∀x∀y(Blind(x) ∧ EqualExcept(x, y, {Blind}) → Tax(t, x) ≤ Tax(t, y))\\ \\ Take a look at the following statement.\\ \\ "An individual with the married filing jointly (MFJ) status with a senior spouse must receive \\ similar or higher tax benefits compared to a similar individual but without the senior spouse."\\ \\ In this case, the first order predicates are: \\ \\ \\ MFJ(x): x is an individual with the married filing jointly status.\\ SeniorSpouse(y): y is a senior spouse of an individual.\\ Tax(t, x): t is the tax paid by individual x.\\ EqualExcept(x, z, S): where x and z are equal individuals except differing only by the predicates in set S.\\ \\ {MFJ(x), SeniorSpouse(y), Tax(t, x), EqualExcept(x, z, S)}\\ \\ Using these predicates, represent the statement in first order logic.\\ \\ \\ Generation Format: you SHOULD ALWAYS generate the first order logic in the following format \\ \\ {your generated first order logic statement} \\ \\ DO NOT generate any other text.\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table*}
